Fast, Small, and Simple Document Listing on Repetitive Text Collections

Document listing on string collections is the task of finding all documents where a pattern appears. It is regarded as the most fundamental document retrieval problem, and is useful in various applications. Many of the fastest-growing string collections are composed of very similar documents, such as versioned code and document collections, genome repositories, etc. Plain pattern-matching indexes designed for repetitive text collections achieve orders-of-magnitude reductions in space. Instead, there are not many analogous indexes for document retrieval. In this paper we present a simple document listing index for repetitive string collections of total length $n$ that lists the $ndoc$ distinct documents where a pattern of length $m$ appears in time $\mathcal{O}(m+ndoc \cdot \log n)$. We exploit the repetitiveness of the document array (i.e., the suffix array coarsened to document identifiers) to grammar-compress it while precomputing the answers to nonterminals, and store them in grammar-compressed form as well. Our experimental results show that our index sharply outperforms existing alternatives in the space/time tradeoff map.

==> tex/img_coll_concat.tex <==
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.49\linewidth}
		\includegraphics[width=\textwidth]{COLL-CONCAT-0010}
%		\caption{10 base documents}
%		\label{fig:gull}
	\end{subfigure}
%	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
	%(or a blank line to force the subfigure onto a new line)
	\begin{subfigure}[b]{0.49\linewidth}
		\includegraphics[width=\textwidth]{COLL-CONCAT-0100}
%		\caption{100 base document}
%		\label{fig:tiger}
	\end{subfigure}

	\caption{
		Document listing on synthetic collection \texttt{Concat}. The $x$ axis shows the total size of the index in bits per symbol. The $y$ axis shows the average time per query in microseconds.
%		We omit the results for the slowest indexes.
	}
	\label{fig:coll_concat}
\end{figure}


==> tex/img_coll_real_breakdown.tex <==
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.4\linewidth}
		\includegraphics[width=\textwidth]{COLL-REAL-BREAKDOWN}
%		\caption{10 base documents}
%		\label{fig:gull}
	\end{subfigure}
%%	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%	%(or a blank line to force the subfigure onto a new line)
%	\begin{subfigure}[b]{0.95\linewidth}
%		\includegraphics[width=\textwidth]{COLL-REVISION-TRADEOFF}
%%		\caption{100 base document}
%%		\label{fig:tiger}
%	\end{subfigure}
%%	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
%	%(or a blank line to force the subfigure onto a new line)
%	\begin{subfigure}[b]{0.95\linewidth}
%	\includegraphics[width=\textwidth]{COLL-INFLUENZA-TRADEOFF}
%	%		\caption{100 base document}
%	%		\label{fig:tiger}
%	\end{subfigure}

	\caption{Size of the main components of the \idxName{GCDA} index on the small real collections. The $y$ axis shows the size in megabytes.
\textcolor{red}{Sacale la palabra "inverted", ponle "Lists of documents"}}
	\label{fig:coll_real_breakdown}
\end{figure}


==> tex/img_coll_version.tex <==
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.49\linewidth}
		\includegraphics[width=\textwidth]{COLL-VERSION-0010}
%		\caption{10 base documents}
%		\label{fig:gull}
	\end{subfigure}
%	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
	%(or a blank line to force the subfigure onto a new line)
	\begin{subfigure}[b]{0.49\linewidth}
		\includegraphics[width=\textwidth]{COLL-VERSION-0100}
%		\caption{100 base document}
%		\label{fig:tiger}
	\end{subfigure}

	\caption{
		Document listing on synthetic collection \texttt{Version}. The $x$ axis shows the total size of the index in bits per symbol. The $y$ axis shows the average time per query in microseconds.
%		We omit the results for the slowest indexes.
	}
	\label{fig:coll_version}
\end{figure}


==> tex/img_nonrep_coll_res.tex <==
\begin{figure*}[t]
	%	\centering
	\begin{subfigure}[b]{0.32\linewidth}
		\includegraphics[width=\textwidth]{COLL-ENWIKI-SMALL}
		%		\caption{small}
		%		\label{fig:gull}
	\end{subfigure}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
	%(or a blank line to force the subfigure onto a new line)
	\begin{subfigure}[b]{0.32\linewidth}
		\includegraphics[width=\textwidth]{COLL-ENWIKI-MID}
		%		\caption{medium}
		%		\label{fig:tiger}
	\end{subfigure}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
	%(or a blank line to force the subfigure onto a new line)
	\begin{subfigure}[b]{0.32\linewidth}
		\includegraphics[width=\textwidth]{COLL-SWISSPROT-SMALL}
		%		\caption{small}
		%		\label{fig:gull}
	\end{subfigure}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
	%(or a blank line to force the subfigure onto a new line)
	%	\begin{subfigure}[b]{0.3\linewidth}
	%		\includegraphics[width=\textwidth]{coll_influenza_small}
	%		\caption{large}
	%		\label{fig:mouse}
	%	\end{subfigure}
	
	\caption{Document listing on non-repetitive collections. The $x$ axis shows the total size of the index in bits per symbol. The $y$ axis shows the average time per query in microseconds.}
	\label{fig:non-repetitive_collections}
\end{figure*}
